Continuity of Functional Transducers: A Profinite Study of Rational Functions

A word-to-word function is continuous for a class of languages~$\mathcal{V}$ if its inverse maps $\mathcal{V}$_languages to~$\mathcal{V}$. This notion provides a basis for an algebraic study of transducers, and was integral to the characterization of the sequential transducers computable in some circuit complexity classes. Here, we report on the decidability of continuity for functional transducers and some standard classes of regular languages. To this end, we develop a robust theory rooted in the standard profinite analysis of regular languages. Since previous algebraic studies of transducers have focused on the sole structure of the underlying input automaton, we also compare the two algebraic approaches. We focus on two questions: When are the automaton structure and the continuity properties related, and when does continuity propagate to superclasses?

==> define.tex <==
\makeatletter

\def\defmath#1#2{\def#1{\ensuremath{#2}\xspace}}
\def\defmathtext#1#2{%
  \edef\@@star{\csname\expandafter\@gobble\string#1 star\endcsname}
  \edef\@@nostar{\csname\expandafter\@gobble\string#1 nostar\endcsname}
  \expandafter\def\@@nostar{\text{\normalfont#2}\xspace}%
  \expandafter\def\@@star{\text{#2}\xspace}%
  \edef#1{%
    \noexpand\protect\noexpand\@ifstar%
    \unexpanded\expandafter{\@@star}
    \unexpanded\expandafter{\@@nostar}}
  }



\defmath\QA{\mathcal{Q\!A}}
\defmathtext\NP{NP}
\defmathtext\DA{\textbf{DA}}
\defmathtext\ACz{AC$^0$}
\defmathtext\NCo{NC$^1$}
\defmathtext\ACCz{ACC$^0$}
\defmathtext\lcm{lcm}
\defmathtext\vA{\textbf{A}}
\defmathtext\TCz{TC$^0$}
\defmath\Msol{\mathcal{M}_{\text{sol}}}
\defmathtext\FACvz{FAC$^0_{\text{v}}$}
\defmathtext\FACCvz{FACC$^0_{\text{v}}$}
\def\resp{resp.\ }
\defmathtext\FACz{FAC$^0$}
\defmath\binal{\{0, 1\}}
\defmath\bbn{\mathbb{N}}
\defmathtext\parity{PARITY}
\defmathtext\even{EVEN}
\defmath\zed{\mathbf{z}}
\defmath\cV{\mathcal{V}}
\defmath\cF{\mathcal{F}}

% \newlength\oneex
% \def\sync{%
%   \mathbin{\text{%
%       \settoheight{\oneex}{x}%
%       \raisebox{0\oneex}{%
%         \resizebox{!}{1.4\oneex}{%
%           \normalsize\tikz{\node [draw,circle,inner sep=0.1em] {\normalfont s};}}}}}}

\def\sync{\bowtie}

% \def\sync{\mathbin{%
%     \tikz[baseline=(char.base)]
%       \node (char) [draw, circle, inner sep =1, scale=0.6]
%          {\footnotesize\normalfont\textrm{sp}};
%        }}
\def\nop{\bullet}
\defmath\cW{\mathcal{W}}
\defmath\cG{\mathcal{G}}
\defmathtext\bV{\textbf{V}}
\defmath\eps{\varepsilon}
\def\reutschu{Reutenauer and Sch{\"u}tzenberger\xspace}
\defmath\taus{\tau_\#}
\defmathtext\REG{REG}
\defmath\mint{\mathsf{MinT}}
\defmath\cts{\mathsf{alph}}
\defmath\Tau{T}
\def\@refpstar#1{(\ref{#1})}
\def\@refpnostar#1{\textit{\@refpstar{#1}}}
\DeclareRobustCommand{\refp}{\@ifstar\@refpstar\@refpnostar}
\def\comp{^{\text{c}}}
\defmathtext\MOD{MOD}
\defmathtext\MAJ{MAJ}
\def\trans#1{\ensuremath{\mathcal{#1}}\xspace}
\def\transT{\trans{T}}
\def\pkh{\mathsf{Pkh}}

\defmath\vJ{\mathcal{J}}

\def\phi{\varphi}
\def\out{\mbox{:}}
\defmathtext\qf{$q_{\text{f}}$}
\defmathtext\rev{${}^{\text{R}}$}

\defmath\vAcom{\mathcal{A}\textit{com}}
\defmath\vA{\mathcal{A}}
\defmath\vDA{\text{$\mathcal{D}$\kern-.14em$\mathcal{A}$}}
\defmath\vR{\mathcal{R}}
\defmath\vL{\mathcal{L}}
\defmath\vG{\mathcal{G}}
\defmath\vGsol{\mathcal{G}_{\text{\normalfont sol}}} % chktex 1
\defmath\vGnil{\mathcal{G}_{\text{\normalfont nil}}} % chktex 1
\defmath\vGp{\mathcal{G}_p}
\defmath\vAb{\text{$\mathcal{A}$\kern-.03em\scalebox{.6}{$\mathcal{B}$}}}
\defmath\vCom{\text{$\mathcal{C}$\kern-0.06em\scalebox{.6}{$\mathcal{O}$\kern-0.1em$\mathcal{M}$}}}
\defmath\Id{\textit{Id}}

\def\@Tif#1,#2,#3\@end{#1_{#2, #3}}
\def\Tif#1{\@Tif#1\@end}
\def\ext#1{\widehat{#1}}
\def\pro#1{\widehat{#1}}
\def\clos#1{\overline{#1}}
\def\equ{\mathsf{Equ}}


% This allows non breaking dashes.
\let\@sb=_
\catcode`_=\active%
\newcommand_{\ifmmode\@sb\else\babelhyphen{nobreak}\fi}



%% |emphasize|.
\let\pipe=|
\catcode`| = 13
\newif\ifemphasize\emphasizefalse%
\def|{\ifmmode\pipe\else%
  \ifemphasize%
    \global\emphasizefalse%
    \egroup%
  \else%
    \global\emphasizetrue%
    \emph\bgroup%
  \fi\fi}



%% Draft related
\def\revisionset! #1 !{\gdef\therevision{#1}} % chktex 26
\def\revision$LastChangedRevision:#1${\revisionset!#1!}

\def\ifzero#1{%
    \@ifnextchar{0}%
      {\expandafter\@firstoftwo\remove@to@nnil}%
      {\expandafter\@secondoftwo\remove@to@nnil}%
        #1\@nnil%
}
\def\ifdraft#1#2{\expandafter\ifzero\expandafter{\the\overfullrule}{#2}{#1}}

\AtBeginDocument{%
  \ifdraft{%
    \let\@@title=\@title%
    \expandafter\gdef\expandafter\@title\expandafter{%
      \expandafter\ooalign\expandafter{\@@title%
        \crcr%
        \hfil%
        \smash{\raisebox{-.3cm}{%
            \normalfont\tiny (rev: \therevision, comp: \today,
                \currenttime)}}%
        \hfil}}}
  {}%
}

%% Probably irrelevant
\usepackage[most]{tcolorbox}
\newenvironment{irr}{\bgroup%
  \footnotesize%
    \begin{tcolorbox}[blanker,left=5mm,
      before skip=6pt,after skip=6pt,
      borderline west={1mm}{0pt}{red},breakable]
      \textit{Probably irrelevant.}\quad
      }{\end{tcolorbox}\egroup}
\def\irrline#1{\begin{irr}#1\end{irr}}


% \DeclareRobustCommand{\qedof}[1]{%
%   \ifmmode \mathqed
%   \else
%     \leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
%     \quad\hbox{\qedsymbol~#1}%
%   \fi
% }

\def\fullstop{\hfill \raisebox{-0.1em}{\tikz\fill (0, 0) rectangle (.82em, .82em);}}
\def\qedof#1{\pushright{\qedsymbol~#1}
    \penalty-700 \par\addvspace{\medskipamount}}

\newenvironment{proofof}[2][\proofname]{\par
  \bgroup%
  \def\qed{\qedof{\itshape of #2\@addpunct{.}}}% % chktex 1
  \begin{proof}[#1]
}{%
\end{proof}
\egroup%
}

\newenvironment{proofnoqed}[1][\proofname]{\par
  \bgroup%
  \def\qed{}
  \begin{proof}[#1]
  }{%
\end{proof}
\egroup%
}

\def\proofstep#1{\par\vspace{.8em}\noindent\emph{(#1.)}\quad}


\tikzstyle{state}=[draw, circle, inner sep=0pt,align=center, text width=5mm]
\tikzstyle{trans}=[bend left, bend angle=5]
\makeatother

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:

